The ETKidney simulator: a discrete event simulator to assess the impact of alternative kidney allocation rules in Eurotransplant

Over 10,000 candidates wait for a kidney transplantation in Eurotransplant, and are prioritized for transplantation based on the allocation rules of the Eurotransplant Kidney Allocation System (ETKAS) and Eurotransplant Senior Program (ESP). These allocation rules have not changed much since ETKAS and ESP's introductions in 1996 and 1999, respectively, despite identification of several areas of improvement by the Eurotransplant Kidney Advisory Committee (ETKAC). A barrier to modernizing ETKAS and ESP kidney allocation rules is that Eurotransplant lacks tools to quantitatively assess the impact of policy changes. We present the ETKidney simulator, which was developed for this purpose. This tool simulates kidney allocation according to the actual ETKAS and ESP allocation rules, and implements Eurotransplant-specific allocation mechanisms such as the system which is used to balance the international exchange of kidneys. The ETKidney simulator was developed in close collaboration with medical doctors from Eurotransplant, and was presented to ETKAC and other major stakeholders. To enhance trust in the ETKidney simulator, the simulator is made publicly available with synthetic data, and is validated by comparing simulated to actual ETKAS and ESP outcomes between 2021 and 2024. We also illustrate how the simulator can contribute to kidney policy evaluation with three clinically motivated case studies. We anticipate that the ETKidney simulator will be pivotal in modernizing ETKAS and ESP allocation rules by enabling informed decision-making on kidney allocation rules together with national competent authorities.

==> tables/coefficients_abdr_matching.tex <==

\begin{tabular}{lllll}
	\toprule
	\multicolumn{1}{c}{ } & \multicolumn{2}{c}{5-year death-censored graft loss} & \multicolumn{2}{c}{10-year death-censored graft loss} \\
	\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5}
	Locus & 1 mismatch & 2 mismatches & 1 mismatch & 2 mismatches\\
	\midrule
	A & 1.07 [0.98-1.16] & \textbf{1.15} [1.01-1.31] & \textbf{1.08} [1.01-1.16] & \textbf{1.15} [1.02-1.28]\\
	B & 1.06 [0.96-1.17] & \textbf{1.28} [1.13-1.44] & 1.08 [0.99-1.18] & \textbf{1.27} [1.15-1.41]\\
	DR & \textbf{1.12} [1.03-1.22] & \textbf{1.35} [1.18-1.55] & \textbf{1.13} [1.05-1.22] & \textbf{1.33} [1.18-1.49]\\
	\bottomrule
\end{tabular}

==> tables/validation/2025-01-09/summary_transplantation_results_ESP.tex <==
\hspace*{-.05\linewidth}
\centering
\begin{tabular}{L{4.9cm} R{5.2cm} L{2cm}}
\toprule
\multirow[b]{1.5}{*}{category} & \multirow[b]{1.5}{*}{\makecell{simulated results\\(average and 95\%-IQR)}} & \multirow[b]{1.5}{*}{\makecell{actual data\\(2021-2024)}}\\
& & \vspace{-0em} \\
\midrule
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{allocation mechanism}}\\
\hspace{1em}standard & \textbf{1117   [-10\%, 1049-1188]} & 1237\\
\hspace{1em}non-standard & \textbf{623    [\Plus23\%, 551-690]} & 508\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{recipient characteristics}}\\
\hspace{1em}pediatric recipient & 0 & 0\\
\hspace{1em}aged 65 or over & \textbf{1512   [-4\%, 1475-1548]} & 1567\\
\hspace{1em}aged below 65 & \textbf{228    [\Plus28\%, 192-261]} & 178\\
\hspace{1em}primary transplant & 1661   [1644-1677] & 1665\\
\hspace{1em}repeat transplant & 80     [67-92] & 80\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{hLA match quality}}\\
\hspace{1em}0 ABDR & 3      [1-6] & 4\\
\hspace{1em}0 or 1 BDR & 62     [50-77] & 55\\
\hspace{1em}1B+1DR or 2B+0DR & 316    [285-348] & 336\\
\hspace{1em}2DR or 3+ BDR & 1360   [1328-1388] & 1350\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{sensitization status}}\\
\hspace{1em}0\% & 1477   [1455-1502] & 1468\\
\hspace{1em}$>$0-84.9\% & 256    [233-278] & 264\\
\hspace{1em}85-94.9\% & 6      [2-10] & 9\\
\hspace{1em}95+\% & \textbf{2      [-50\%, 1-3]} & 4\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{match geography}}\\
\hspace{1em}Austria & 106    [87-128] & 118\\
\hspace{1em}Belgium & 107    [83-132] & 120\\
\hspace{1em}Croatia & 38     [26-51] & 26\\
\hspace{1em}Germany & \textbf{1081   [\Plus3\%, 1049-1118]} & 1048\\
\hspace{1em}Hungary & 19     [11-28] & 24\\
\hspace{1em}Netherlands & 380    [349-406] & 398\\
\hspace{1em}Slovenia & 9      [4-15] & 11\\
\hspace{1em}local/regional & 1374   [1324-1424] & 1408\\
\hspace{1em}interregional & 174    [138-206] & 178\\
\hspace{1em}international & 192    [153-225] & 159\\
\bottomrule
\end{tabular}


==> tables/validation/2025-01-09/summary_transplantation_results_ETKAS.tex <==
\hspace*{-.05\linewidth}
\centering
\begin{tabular}{L{4.9cm} R{5.2cm} L{2cm}}
\toprule
\multirow[b]{1.5}{*}{category} & \multirow[b]{1.5}{*}{\makecell{simulated results\\(average and 95\%-IQR)}} & \multirow[b]{1.5}{*}{\makecell{actual data\\(2021-2024)}}\\
& & \vspace{-0em} \\
\midrule
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{allocation mechanism}}\\
\hspace{1em}standard & 5044   [4881-5169] & 5000\\
\hspace{1em}non-standard & 761    [632-915] & 804\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{recipient characteristics}}\\
\hspace{1em}pediatric recipient & 339    [321-358] & 325\\
\hspace{1em}aged 65 or over & 734    [700-769] & 725\\
\hspace{1em}aged below 65 & 5071   [5034-5105] & 5079\\
\hspace{1em}primary transplant & 5038   [5001-5068] & 5039\\
\hspace{1em}repeat transplant & 768    [734-795] & 765\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{hLA match quality}}\\
\hspace{1em}0 ABDR & \textbf{650    [\Plus5\%, 624-675]} & 617\\
\hspace{1em}0 or 1 BDR & 1136   [1083-1179] & 1153\\
\hspace{1em}1B+1DR or 2B+0DR & 2468   [2406-2534] & 2492\\
\hspace{1em}2DR or 3+ BDR & 1551   [1490-1609] & 1542\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{sensitization status}}\\
\hspace{1em}0\% & \textbf{4211   [\Plus2\%, 4173-4255]} & 4142\\
\hspace{1em}$>$0-84.9\% & 1320   [1279-1356] & 1355\\
\hspace{1em}85-94.9\% & 173    [155-191] & 186\\
\hspace{1em}95+\% & \textbf{101    [-17\%, 87-114]} & 121\\
\addlinespace[0.3em]
\multicolumn{3}{l}{\textbf{match geography}}\\
\hspace{1em}Austria & 532    [525-538] & 530\\
\hspace{1em}Belgium & 912    [905-918] & 914\\
\hspace{1em}Croatia & \textbf{277    [\Plus3\%, 272-283]} & 270\\
\hspace{1em}Germany & 2648   [2635-2659] & 2651\\
\hspace{1em}Hungary & \textbf{464    [-2\%, 457-470]} & 472\\
\hspace{1em}Netherlands & 854    [847-860] & 849\\
\hspace{1em}Slovenia & 119    [113-124] & 118\\
\hspace{1em}local/regional & \textbf{4087   [\Plus5\%, 3993-4164]} & 3902\\
\hspace{1em}interregional & \textbf{637    [-11\%, 590-680]} & 715\\
\hspace{1em}international & \textbf{1081   [-9\%, 1012-1164]} & 1187\\
\bottomrule
\end{tabular}

